Understanding Data Storage and Ingestion for Large-Scale Deep Recommendation Model Training

Datacenter-scale AI training clusters consisting of thousands of domain-specific accelerators (DSA) are used to train increasingly-complex deep learning models. These clusters rely on a data storage and ingestion (DSI) pipeline, responsible for storing exabytes of training data and serving it at tens of terabytes per second. As DSAs continue to push training efficiency and throughput, the DSI pipeline is becoming the dominating factor that constrains the overall training performance and capacity. Innovations that improve the efficiency and performance of DSI systems and hardware are urgent, demanding a deep understanding of DSI characteristics and infrastructure at scale. This paper presents Meta's end-to-end DSI pipeline, composed of a central data warehouse built on distributed storage and a Data PreProcessing Service that scales to eliminate data stalls. We characterize how hundreds of models are collaboratively trained across geo-distributed datacenters via diverse and continuous training jobs. These training jobs read and heavily filter massive and evolving datasets, resulting in popular features and samples used across training jobs. We measure the intense network, memory, and compute resources required by each training job to preprocess samples during training. Finally, we synthesize key takeaways based on our production infrastructure characterization. These include identifying hardware bottlenecks, discussing opportunities for heterogeneous DSI hardware, motivating research in datacenter scheduling and benchmark datasets, and assimilating lessons learned in optimizing DSI infrastructure.

==> Makefile <==
TEX_SOURCES=$(shell ls *.tex)
ALL_FIGS=$(shell find figures -type f)

all: paper.pdf

view: paper.pdf
	open paper.pdf

RERUN=egrep -q '(^LaTeX Warning:|\(natbib\)).* Rerun' paper.log

paper.pdf: ${TEX_SOURCES} figures
	pdflatex -interaction=nonstopmode paper.tex
	bibtex -min-crossrefs=1000 paper
	pdflatex -interaction=nonstopmode paper.tex
	pdflatex -interaction=nonstopmode paper.tex
	while ( $(RERUN) ); do pdflatex paper.tex; done

figures: $(ALL_FIGS)

clean:
	rm -rf *.aux *.bbl *.blg *.log *.out *.synctex.gz *.fls *.fdb_latexmk paper.pdf

# The following target is useful for debugging Makefiles; it
# prints the value of a make variable.
print-%:
	@echo $* = $($*)

.PHONY: figures clean all view

.PRECIOUS:
.SECONDARY:


==> fig-fault-tolerance.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=2.5in]{figures/fault_tolerance.png}
  \caption{\small Breakdown of successful jobs, failed jobs (due to DPP and other factors), and jobs saved by DPP fault tolerance over a one week period.}
  \label{fig:fault_tolerance}
  \vspace{-3mm}
\end{figure}


==> fig-feature-flattening.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/feature-flattening.png}
  \caption{\small Feature Flattening example}
  \label{fig:feature-flattening}
\end{figure}


==> fig-feature-regrouping.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/feature-regrouping.png}
  \caption{\small Feature Regrouping example}
  \label{fig:feature-regrouping}
\end{figure}


==> fig-flatmap.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/flatmap.png}
  \caption{\small Worker throughput and percent improvement across number of Worker threads as in-memory flatmaps are applied.}
  \label{fig:flatmap}
\end{figure}


==> fig-functional-bd.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/functional_dsi_bd.pdf} 
  \caption{\small Functional view of the DSI pipeline. Throughput demands are driven by the trainers.}
  \vspace{-3mm}
  \label{fig:functional_bd}
\end{figure}


==> fig-gang-size.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/gang_size.png}
  \caption{\small Normalized histogram of number of \SystemName workers used across jobs over 90 days. \SystemName meets diverse preprocessing demands.}
  \label{fig:gang_size}
  \vspace{-3mm}
\end{figure}


==> fig-model-complexity.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/model_complexity.png}
  \caption{\small Projected growth in model throughput of RM1 in the next three years.}
  \label{fig:model_complexity}
\end{figure}


==> fig-recommendation-model.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/recommendation_model.pdf} 
  \caption{\small Model architecture for deep recommendation model}
  \label{fig:recommendation_model}
\end{figure}


==> fig-regrouping.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/regrouping_bar.png}
  \caption{\small Reduction in Storage Throughput and Payload Size overheads from storage due to feature reordering.}
  \label{fig:regrouping}
\end{figure}


==> fig-stripe-size.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=3.33in]{figures/stripe_sizes.png}
  \caption{\small Reduction in storage throughput overhead, normalized to optimal reordering, due to production-reordering and increased stripe sizes. Spark's default stripe size is the left-most point.} %
  \vspace{-3mm}
  \label{fig:stripe_size}
\end{figure}


==> tbl-fault-tolerance.tex <==
\begin{table}[t]
  \centering
  \footnotesize
\begin{tabular}{@{}lll@{}}
\toprule
\% Successful Jobs & \% Jobs Saved with FT & \% Jobs Failed \\ \midrule
66.13              & 24.25                 & 9.61           \\ \bottomrule
\end{tabular}%
\caption{\small Percent of successful, saved, and failed GPU training jobs over a one week period.}
  \label{tbl:fault_tolerance}
  \vspace{-2mm}
\end{table}


==> tbl-feature-flattening.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \caption{\small Throughput gain due to reduced extraction CPU cycles, and increased storage overhead, with feature flattening for $RM_1$.}%
  \label{tbl:feature_flattening}
  \vspace{-3mm}
  \begin{tabular}{@{}llll@{}}
    \toprule
    Experiment         & \thead{Normalized \\ Reader Throughput} & \thead{\% CPU Cycles \\ on Extraction} & \thead{Storage Size \\ Overhead}  \\ \midrule
    Baseline           & 1.00                         & 63                & 1.00 \\
    Feature Flattening & 2.00                         & 42                & 1.12 \\ \bottomrule
  \end{tabular}
  \vspace{-4mm}
\end{table}



==> tbl-flash-power.tex <==
\begin{table}[t]
  \centering
  \footnotesize
\begin{tabular}{@{}llll@{}}
\toprule
Storage Architecture   & HDD Power & SSD Power & Power Savings \\ \midrule
HDD (R=3)              & 1         & -         & -             \\
HDD (R=3); SSD (R=1)   & 0.15      & 0.52      & 34            \\
HDD (R=3); SSD (Cache) & 0.15      & 0.26      & 59            \\ \bottomrule
\end{tabular}%
\caption{\small Normalized power requirements and savings across storage architectures.}
  \label{tbl:flash_power}
\end{table}


==> tbl-llc-miss.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{\small Attribution of LLC misses during preprocessing for $RM_2$.}\label{tbl:llc-miss}
\begin{tabular}{@{}lllll@{}}
\toprule
                 & Transformations & Reading & Network RX & Network TX \\ \midrule
\% of LLC Misses & 50.4            & 24.9    & 16.4       & 4.7        \\ \bottomrule
\end{tabular}%
\end{table}

==> tbl-optimizations.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
  \begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.4\linewidth}|p{0.4\linewidth}|}
    \toprule
    Design & Pipeline Component & Summary & Impact \\ \hline
    Disaggregation &
    DPP &
    Run data reading and preprocessing on distributed nodes. &
    Allow right-sizing of readers to trainer throughput requirements, avoiding data stalls. \\ \hline
    Fault Tolerance &
    DPP &
    DPP workers checkpoint reader state. &
    Recovers from frequent reader faults that cause training jobs to fail. \\ \hline
    Feature Flattening &
    Warehouse &
    Store feature values across rows in a stream. &
    Allow storage nodes to selectively send only used feature streams. \\ \hline
    Flatmaps &
    DPP &
    Modify DPP in-memory data structure to allow easy indexing of data by feature &
    Reduce overheads at reader to transform raw feature bytes to tensors. \\ \hline
    Feature Regrouping &
    Warehouse &
    Group features that are frequently read by a model together in storage. &
    Reduce over-reading blocks of data from storage. \\ \hline
  \end{tabular}
  \caption{\small Optimizations across the data ingestion pipeline.}
  \label{tbl:optimizations}
\end{table*}


==> tbl-storage-skus.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \begin{tabular}{@{}lll@{}}
    \toprule
    Server Type & Norm. Storage per Watt & Norm. Read BW per Watt \\ \midrule
    HDD         & 1.00                        & 1.00                          \\
    SSD         & 0.09                        & 3.26                          \\ \bottomrule
  \end{tabular}%
  \caption{\small Normalized storage capacity and read bandwidth per watt for our HDD and SSD storage nodes.}
  \label{tbl:storage_skus}
  \vspace{-3mm}
\end{table}

